Unknotting numbers of 2-spheres in the 4-sphere

We compare two naturally arising notions of unknotting number for 2-spheres in the 4-sphere: namely, the minimal number of 1-handle stabilizations needed to obtain an unknotted surface, and the minimal number of Whitney moves required in a regular homotopy to the unknotted 2-sphere. We refer to these invariants as the stabilization number and the Casson-Whitney number of the sphere, respectively. Using both algebraic and geometric techniques, we show that the stabilization number is bounded above by one more than the Casson-Whitney number. We also provide explicit families of spheres for which these invariants are equal, as well as families for which they are distinct. Furthermore, we give additional bounds for both invariants, concrete examples of their non-additivity, and applications to classical unknotting number of 1-knots.

==> macros.tex <==

\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\theoremstyle{definition}
\newtheorem*{convention}{Conventions}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{question}{Question}[section]

\makeatletter
\let\c@conjecture=\c@theorem
\let\c@corollary=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@definition=\c@theorem
\let\c@example=\c@theorem
\let\c@remark=\c@theorem
\let\c@observation=\c@theorem
\let\c@question\c@theorem
\makeatother

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
\makeautorefname{theorem}{Theorem}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{definition}{Definition}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%

\numberwithin{equation}{section}

\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
\newlength\fcaph
\newlength\fdesc
\newlength\factualfontsize
\settoheight{\fcaph}{\footnotesize \Alphabet}
\settodepth{\fdesc}{\footnotesize \Alphabet \alphabet}
\setlength{\factualfontsize}{\dimexpr\fcaph+\fdesc\relax}

\newcommand{\bit}[1]{\textbf{\textit{#1}}}
\newcommand{\cs}{\mathop\#}

% Orange placeholder for reference to
% a figure that is to be made
\newcommand{\Pic}{\textcolor{orange}{[Pic]}}

% Typesetting for a 'big' quotient
% from
% https://tex.stackexchange.com/questions/4624/a-symbol-for-the-quotient-of-two-objects/4625
\newcommand{\bigslant}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}

% Comments
\numberwithin{equation}{section}
\newcounter{commentcounter}
\newcommand{\commentb}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by B.)}:
	{\textcolor{blue}{#1}} }
\newcommand{\commentj}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by J.)}:
	{\textcolor{purple}{#1}} }
\newcommand{\commenth}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by H.)}:
	{\textcolor{green}{#1}} }
\newcommand{\commentm}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by M.)}:
	{\textcolor{orange}{#1}} }
